An Adaptive Clustering Approach for Accident Prediction

Traffic accident prediction is a crucial task in the mobility domain. State-of-the-art accident prediction approaches are based on static and uniform grid-based geospatial aggregations, limiting their capability for fine-grained predictions. This property becomes particularly problematic in more complex regions such as city centers. In such regions, a grid cell can contain subregions with different properties; furthermore, an actual accident-prone region can be split across grid cells arbitrarily. This paper proposes Adaptive Clustering Accident Prediction (ACAP) - a novel accident prediction method based on a grid growing algorithm. ACAP applies adaptive clustering to the observed geospatial accident distribution and performs embeddings of temporal, accident-related, and regional features to increase prediction accuracy. We demonstrate the effectiveness of the proposed ACAP method using open real-world accident datasets from three cities in Germany. We demonstrate that ACAP improves the accident prediction performance for complex regions by 2-3 percent points in F1-score by adapting the geospatial aggregation to the distribution of the underlying spatio-temporal events. Our grid growing approach outperforms the clustering-based baselines by four percent points in terms of F1-score on average.

==> ITSC_2021 _AccidentPrediction/table-regions.tex <==

\begin{table}[htbp]
    \centering
    \caption{F1-score of accident predictions of different cities with different aggregations
    }
    \small{
    % \renewcommand{\arraystretch}{.95}
    \begin{tabular}{ll c c c c c c}
    \toprule
         Clustering & Method & Hannover & Munich & Nuremberg  \\
         \midrule
        Grid-Growing    & \approach{} &  \textbf{0.58}& \textbf{0.56}&\textbf{0.60}   \\
        Grid-Growing    & DAP &0.47  &0.44 &  0.47  \\
        Grid-Growing    & DNN & 0.55 &0.52 &0.54    \\
        Grid-Growing    & LR & 0.56 & 0.49&  0.53  \\
        Grid-Growing    & GBC & 0.52 & 0.52&0.56    \\
        \midrule
        SOM    & \approach{} &\textbf{0.56}  & \textbf{0.55} & \textbf{0.57}   \\
        SOM    & DAP & 0.42 &0.44 &   0.45 \\
        SOM    & DNN & 0.51 &0.51 &  0.54  \\
        SOM    & LR & 0.53 &0.46 &  0.53  \\
        SOM    & GBC &  0.52&0.51 & 0.54   \\
        \midrule
         1x1    & \approach{} & \textbf{0.59} & \textbf{0.57} & \textbf{0.60}  \\
        1x1    & DAP &  0.49& 0.49& 0.51   \\
        1x1    & DNN &  0.57& 0.52&  0.57  \\
        1x1    & LR &  0.57&0.52 &  0.57  \\
        1x1    & GBC &  0.52&0.51 & 0.55   \\
        \midrule
        5x5    & \approach{} & \textbf{0.52} &\textbf{0.51} &  \textbf{0.53} \\
        5x5    & DAP & 0.45 &0.44 &  0.45  \\
        5x5    & DNN &  0.50& 0.49&  0.51  \\
        5x5    & LR & 0.49 &0.40 & 0.48   \\
        5x5    & GBC &  0.16&0.26 & 0.18   \\
        %  \approach{}+DBSCAN & 0.70/147 &0.60/63 & 0.63/32&0.667/72 &0.66/45 & 0.748/918   \\
        %  DAP &0.488  &0.53 &0.449 &0.44 & 0.65&0.61 \\ %5x5 Grid
        %  DNN &0.49  & 0.59& 0.549& 0.548&0.64 & 0.607\\
        %  LR &0.35 &0.60 &0.56 &0.59 &0.62 &0.53  \\
        %  GBC &0.45 & 0.602&0.53 & 0.60&0.586 & 0.58\\
         \bottomrule
    \end{tabular}
    }
    \label{tab:regions}
\end{table}
